When does mixup promote local linearity in learned representations?

Mixup is a regularization technique that artificially produces new samples using convex combinations of original training points. This simple technique has shown strong empirical performance, and has been heavily used as part of semi-supervised learning techniques such as mixmatch~\citep{berthelot2019mixmatch} and interpolation consistent training (ICT)~\citep{verma2019interpolation}. In this paper, we look at Mixup through a \emph{representation learning} lens in a semi-supervised learning setup. In particular, we study the role of Mixup in promoting linearity in the learned network representations. Towards this, we study two questions: (1) how does the Mixup loss that enforces linearity in the \emph{last} network layer propagate the linearity to the \emph{earlier} layers?; and (2) how does the enforcement of stronger Mixup loss on more than two data points affect the convergence of training? We empirically investigate these properties of Mixup on vision datasets such as CIFAR-10, CIFAR-100 and SVHN. Our results show that supervised Mixup training does not make \emph{all} the network layers linear; in fact the \emph{intermediate layers} become more non-linear during Mixup training compared to a network that is trained \emph{without} Mixup. However, when Mixup is used as an unsupervised loss, we observe that all the network layers become more linear resulting in faster training convergence.

==> legacy.tex <==
We now explain the use of mixup operation (\eqref{eq:mixup_op}) in semi-supervised learning techniques and how it effects the linearity of network representations.

\paragraph{Interpolation Consistency Training (ICT)}
Mixup operation can be used with unlabelled examples to perform unsupervised representation learning. 
%
\citet{verma2019interpolation} proposed to use mixup with two unlabelled examples such that the network predictions ($f_{\param}$) remain consistent on the mixed up example and mixed up representations of individual examples.
%
More specifically, for two unlabeled examples $u_1$ and $u_2$, they learn a function $f_{\param}$ such that:
%
$$f_\param(\mixop(u_1, u_2)) \approx \mixop(f_\param(u_1), f_\param(u_2)).$$
%
%\ie the prediction at the convex combination of the examples, and the convex combination of the predictions at the examples remain similar. 
%[Arslan - fixed in the setup]\sj{We should define exactly what $f_\theta$ is. For example, does it output logits or probabilities?}:

In the remainder, we omit $\param$ from $f(\cdot)$ to simplify the notation.
%
This objective can easily be incorporated in the form of an unsupervised loss in the network training:
\begin{equation} \label{eq:ict2}
    %\usuploss = \biggl( f(\mixop(u_1, u_2)) - \mixop(f(u_1), f(u_2)) \biggr)^2
    \usuploss = D\biggl( f(\mixop(u_1, u_2)) , \mixop(f(u_1), f(u_2)) \biggr)
\end{equation}
%
where $D$ is a distance measure in some space (\eg) L2-distance in Euclidean space or KL-divergence in Riemannian space.
%
In the remainder, we use L2 as the distance measure unless stated otherwise.
%
This loss is referred to as Interpolation Consistency Training (ICT) loss~\citep{verma2019interpolation}. 

The authors~\citep{verma2019interpolation} argued that ICT helps in semi-supervised learning as it effectively enforces the so-called {\em consistency regularization}, whereby the predictions remain unchanged when an input $u$ is perturbed by a small amount $\delta$, \ie $f(u) \approx f(u+\delta)$. 
%
Consistency regularization forces the model's decision boundary to traverse a low-density path, \ie, a path where the training data is low, which is found to be an effective learning signal studied in many semi-supervised learning techniques \citep{sajjadi2016regularization,laine2016temporal,tarvainen2017mean,miyato2018virtual}.

\paragraph{Linearity}
%
Mixup operation, as used in the ICT loss (\eqref{eq:ict2}) or supervised losses elsewhere~\citep{Zhang2017}, can be seen as a way to make the network $f(\cdot)$ more linear.
%
Recent works~\citep{verma2019manifold,guo2019mixup,carratino2020mixup,zhang2020does} have shown that forcing the network function $f(\cdot)$ to behave linearly on the convex combination of pairs of inputs and corresponding labels (if supervised loss is used), leads to better generalization.
%mixup regularization~\citep{Zhang2017}, that forces the network predictions to behave linearly for the convex combination of pairs of inputs, leads to better generalization \citep{verma2019manifold,guo2019mixup,carratino2020mixup,zhang2020does} . 
%
\citet{carratino2020mixup} and \citet{zhang2020does} argued that this generalization comes from the regularized Jacobian of the network that is induced by the mixup operation. 

In this work, we empirically study the effect of mixup operation on the network training.
Towards this, we first study how the linearity enforced on the network predictions by the mixup regularization, effects the representations learned in the intermediate network layers \ie, whether the intermediate layers become more or less linear during network training. 
%
We measure the nonlinearity of a layer `$l$' on a held out dataset $\dataset_{te}$ at the $t$-th training step by:
\begin{equation} \label{eq:linearity}
\begin{split}
    \linmsr_t(l) = \sum_{(x_1, x_2) \sim \dataset_{te}} D\biggl(&\hat{f}^{l}_t(\mixop(x_1, x_2)) - \\
    &\mixop(\hat{f}^{l}_t(x_1), \hat{f}^{l}_t(x_2)) \biggr), 
\end{split}
\end{equation}
%
where $\hat{f}^l_t(\cdot)$ is the output of layer $l$ at the $t$-th iteration of the SGD. 
%
The output is constrained to have a unit norm \ie $\hat{f}^l_t= \frac{f^l_t}{\|f^l_t\|}$, to compare the nonlinearity across different layers. \sj{Should we not also normalize \eqref{eq:linearity} by the size of $\dataset_{te}$?}

We then study the effect of using more mixup points to, arguably, enforce stronger linearity in the last layer and its influence on network convergence in terms of both labeled samples and training steps.  
%
Formally, we extend the ICT regularization (\eqref{eq:ict2}) to a K-simplex. 
%
We define an unsupervised loss on a set of K unlabeled points, $\ictset~=~\{u_1, \cdots, u_K\}$, as:
\begin{equation} \label{eq:ictx}
    \ictx_K = D\biggr( f\bigl(\mixop(\ictset)\bigr) - \mixop\bigl(f(u_1), \cdots, f(u_K)\bigr) \biggr), 
\end{equation}
%
where $\mixop(\ictset)$ is the mixup operation, as defined in \eqref{eq:mixup_op}, on the set $\ictset$.

\subsection{Propagation of linearity to intermediate layers} \label{sec:linear_propag}



We first look at the effect of mixup-based regularization on the linearity of intermediate layers in both supervised and semi-supervised setups. 
%
\paragraph*{Experimental setup}
We use the standard semi-supervised learning datasets; CIFAR-10, CIFAR-100, and SVHN.
%
For the results in this section, we use a ResNet-52 architecture \citep{he2016deep}.
%
We refer to ResNet blocks as stages (numbered from 1 to 6 with `1' being the block closest to input and `6' being the classification layer). 
%
The batch size is set to $128$ and Adam optimizer~\citep{kingma2014adam} (learning rate = $0.002$, $\beta_1$ = 0.9, $\beta_2$ = 0.999) is used. 
%
The $\alpha$ for the Dirichlet distribution is set to $0.5$ for CIFAR-10 and CIFAR-100, and $0.1$ for SVHN dataset.
%
The total training steps are kept fixed for all datasets and for all labeled dataset sizes ($|\dataset_s|$). 
%
Each method is run with $5$ different random seeds and the performance is averaged across these runs, and error bars are reported. 

\Figref{fig:main_linearity_prop} shows the nonlinearity computed in different network stages throughout the network training for different values of $K$ in the ICT loss (\eqref{eq:ictx}).
%
The results here are reported on CIFAR-10 and SVHN datasets (refer to supplementary for CIFAR-100 results).
%
For the \textbf{supervised case} (ERM and mixup), it can be seen from the figure that {\em different network stages generally remain nonlinear.} 
%
Specifically, for ERM the last stage is always highly nonlinear, whereas for mixup it is strongly linear. 
%
However, we observe an interesting interplay of nonlinearities in the stages preceding the last stage. 
%
For the ERM, the second last stage (stage 4) is highly linear, whereas for mixup it is highly nonlinear. 
%
Similarly, the stages $2$ and $3$ are relatively more nonlinear for mixup than they are for the ERM. 
%
Finally, stages $0$ and $1$ are more linear for mixup.
%
This interplay of nonlinearities for the ERM and mixup in different layers suggests that the stronger linearity enforced by the supervised mixup loss~\citep{Zhang2017} in the last layer comes at the cost of making the preceding layers strongly nonlinear.  
\sr{Can we really say that it makes the previous layers more nonlinear than what we observe without mixup? Or is it just that the nonlinearity is not affected by the enforcement on mixup loss on the last layer?} The network tries to preserve the overall nonlinearity from input to output and accounts for a strong linearity in one layer by a strong nonlinearity in the other layers. 

For the \textbf{semi-supervised case} ($\ictx_K$), when the linearity is enforced on the network predictions, with the help of the ICT loss (\eqref{eq:ictx}) on a large unlabeled dataset, we observe that all the network layers remain relatively more linear compared to the supervised case. 
%
Furthermore, the stronger the ICT loss (large $K$), the more linear the network stages are. 
% 
Contrary to the supervised case, where the linearity in the last stage reflected in the strong nonlinearity in the preceding stages (or vice versa), the semi-supervised training with ICT loss tends to make all stages linear. 
%
\sr{%
Develop a theoretical argument around as to why this happens. 
}


\sr{There is a difference between the linearity enforced in supervised and semi-supervised cases. In supervised cases, we are only taking a convex combination of sparse one-hot vectors, whereas in the semi-supervised cases we are taking the convex combination of dense vectors. In supervised case, we fix the groundtruth predictions. In semi-supervised case, the pseudo-labels can evolve and change. At a high level, the semi-supervised loss seems to be a much stronger regularization than the supervised loss.}

\todo{%
This suggests that semi-supervised training with ICT loss makes the overall function $f(\cdot)$ more smooth. 
%
We empirically verify this by computing the empirical Lipschitz constant \footnote{Defined as $\lip_2(f) = \max_{(x_i, x_j) \in \dataset_{te}}\frac{||f(x_i) - f(x_j)||_{2}}{||x_i - x_j||_2}$, for 2-norm.} of the trained network.
%
Specifically, once the network is trained to convergence, we sample $200$ pairs from $\dataset_{te}$ and compute the average empirical Lipschitz across these pairs \ie, $\lip_2 = \frac{1}{200} \sum_{(x_1, x_2) \in \dataset_{te}} \frac{||f(x_1) - f(x_2)||_{2}}{||x_1 - x_2||_2}$.
%
We record the results in Table X.} 

\sr{Computing the empirical Lipshitz constant sounds like a good thing to try.}


\subsection{Effect of linearity on network convergence} \label{sec:strong_linear}

\begin{figure*}[t]
	\begin{minipage}[t]{0.45\textwidth}
        \begin{center}
                \includegraphics[scale=0.55]{plots/mixmatch_ictX/cifar10.pdf}\\
                 {\small CIFAR-10}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{0.55\textwidth}
        \begin{center}
                \includegraphics[scale=0.55]{plots/mixmatch_ictX/svhn.pdf}\\
                 {\small SVHN}
        \end{center}
        \end{minipage}%
\caption{Test accuracy when stronger linearity is enforced. ERM and mixup refer to the cases where only supervised loss is used. $\ictx_K$ refer to a setup where the ICT loss with $K$ mixup points are used as unsupervised loss. The supervised loss with the ICT does not use mixup loss.}
\label{fig:ictX}
\end{figure*}

We now analyze the effect of mixup-based regularization on network convergence in both labeled samples and training steps. 
%
The experimental setup in this section follows that of the previous section.

We first look at the convergence in the labeled samples. 
%
\Figref{fig:ictX} shows the performance on CIFAR-10 and SVHN datasets for various sizes of the labeled dataset.
%
It can be seen from the figure that when the size of the labeled dataset is very small, enforcing a stronger linearity on the network predictions, with the help of ICT loss on a large unsupervised dataset, leads to significantly better performance. 
%
For example, in CIFAR-10 and with 250 labeled examples, the performance improves from $47.5 (\pm 2.69)$\% to $69.9 (\pm 3.72)$\% when $2$ and $5$ points are used in the ICT loss (\eqref{eq:ictx}), respectively. 
% 
A similar trend can also be seen in the SVHN dataset.
%
Another way of looking at the same figure is that to achieve a performance of $\sim 70$\% on the test set of CIFAR-10, $\ictx_2$ requires roughly $1000$ labeled samples, whereas $\ictx_5$ requires only $250$ labeled samples. 
%
In this sense, we say that $\ictx_5$ converges faster (in terms of labeled samples) to the desirable performance than $\ictx_2$. 
%
However, as the size of the labeled dataset increases, all methods converge to the same accuracy as per the expectation.

We now look at the convergence in the training steps. 
%
\todo{We need to show that under the same experimental setup as that of the previous section, $\ictx_K$ converges faster for large values of $K$.}

To further understand the effect of stronger enforcement of linearity, we visualize the decision boundaries of the classifiers, trained in a semi-supervised setup, in controlled experiments. 
%
Specifically, we train classifiers in a semi-supervised setup on 2-way and 3-way classification tasks and plot the results in \figref{fig:ictx_convergence}. 
%
It can be seen from the figure that, as described by \citet{verma2019interpolation}, ICT allows the classifier to traverse a low density region. 
%
Furthermore, and more importantly to our analysis, the stronger enforcement of ICT loss by using more unlabeled points (\eqref{eq:ictx}), ICT recovers the decision boundaries in fewer training steps. 
%
For example, for both the 2-way and 3-way classification, $\ictx_3$ recovers the same decision boundary in $5$k SGD steps that take $\ictx_2$ $10$k steps. 
%
Further results on 2-, 3-, and 4-way classification tasks with different data distributions are shown in the supplementary.
%
This further supports our hypothesis that the stronger enforcement of linearity, by means of mixup-based unsupervised losses, allows the model to converge quickly in training steps. 
%
\todo{Perhaps, we should also show the convergence in labeled samples on these toy setups.}

\begin{figure*}[t]
        \def \MINPAGE {0.25}
        \def \FIGSCALE {0.32}
        
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/convergence/fullysup_2moons.png}\\
                 {\small Ideal (fully supervised), $5$k steps}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/convergence/sup_2moons.png}\\
                 {\small ERM ($\dataset_s$ only), $10$k steps}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/convergence/ict2_2moons.png}\\
                 {\small $\ictx_2$ ($\dataset_s \cup \dataset_{us}$), $10$k steps}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/convergence/ict3_2moons.png}\\
                {\small $\ictx_3$ ($\dataset_s \cup \dataset_{us}$), $5$k steps}
        \end{center}
        \end{minipage}
        
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/convergence/fullysup_3moons.png}\\
                 {\small Ideal (fully supervised), $5$k steps}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/convergence/sup_3moons.png}\\
                 {\small ERM ($\dataset_s$ only), $10$k steps}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/convergence/ict2_3moons.png}\\
                 {\small $\ictx_2$ ($\dataset_s \cup \dataset_{us}$), $10$k steps}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/convergence/ict3_3moons.png}\\
                {\small $\ictx_3$ ($\dataset_s \cup \dataset_{us}$), $5$k steps}
        \end{center}
        \end{minipage}
        
\caption{Classifier decision boundary on 2-way (top row) and 3-way (bottom row) classification tasks. Ideal refers to a fully supervised setup when the labels are known for both the $\dataset_s$ and $\dataset_{us}$. The solid dots are labeled points ($\dataset_s$). $\ictx_3$ recovers the decision boundary in the least training steps.}
\label{fig:ictx_convergence}
\end{figure*}

\subsection{Effect of labeled examples} \label{sec:labeled_examples}

\begin{figure*}[t]
        \def \MINPAGE {0.25}
        \def \FIGSCALE {0.32}
        
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/toysetup/moons2/ict2_nclusters4_npoints2_samplingConc.pdf}\\
                 {\small $\ictx_2$}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/toysetup/moons2/ict2_nclusters4_npoints2_samplingKMeans.pdf}\\
                 {\small $\ictx_2$}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/toysetup/moons2/ict3_nclusters4_npoints2_samplingConc.pdf}\\
                 {\small $\ictx_3$}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/toysetup/moons2/ict3_nclusters4_npoints2_samplingKMeans.pdf}\\
                {\small $\ictx_3$}
        \end{center}
        \end{minipage}
        
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/toysetup/moons2/ict2_nclusters4_npoints3_samplingRandom.pdf}\\
                 {\small $\ictx_2$}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/toysetup/moons2/ict2_nclusters4_npoints3_samplingKMeans.pdf}\\
                 {\small $\ictx_2$}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/toysetup/moons2/ict3_nclusters4_npoints3_samplingRandom.pdf}\\
                 {\small $\ictx_3$}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/toysetup/moons2/ict3_nclusters4_npoints3_samplingKMeans.pdf}\\
                {\small $\ictx_3$}
        \end{center}
        \end{minipage}
        
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/convergence/ict2_3moons_conc.png}\\
                 {\small $\ictx_2$}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/convergence/ict2_3moons.png}\\
                 {\small $\ictx_2$}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/convergence/ict3_3moons_conc.png}\\
                 {\small $\ictx_3$}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/convergence/ict3_3moons.png}\\
                {\small $\ictx_3$}
        \end{center}
        \end{minipage}
        
\caption{Effect of labeled samples on the classifier decision boundaries. Tow two rows are for a 2-way classification task whereas the third two is for a 3-way classification task. The solid dots refer to the labeled samples. For a 2-way classification, $\ictx_k$ needs at least 3 samples to recover a decision boundary. In all cases, the recovered decision boundaries depend on the choice of labeled samples.}
\label{fig:ictx_sampling}
\end{figure*}

Finally, we try to understand the effect of labeled samples on the recovered decision boundaries for the ICT-based semi-supervised models. 
%
Specifically, we want to look at whether the recovered decision boundaries depend on the number and diversity of labeled samples. 
%
In this section, we will use a similar controlled setup as used in the previous section. 

\Figref{fig:ictx_sampling} shows the classifier decision boundaries for various sizes and sampling strategies of the labeled set.
%
First, from the top row of the figure, it can be seen that, in the 2-way classification task and with only two labeled samples, it is not possible to recover the decision boundary irrespective of the choice of labeled samples and strength of the ICT regularizer (both $\ictx_2$ and $\ictx_3$ fail in this case). 
%
However, in the same 2-way setup and with 3 labeled points, it is possible to recover a decision boundary that traverses a low density path. 
%
This shows that to recover the decision boundary with ICT, a minimum number of labeled points are required. 
%
\ac{Can we develop a bound on the samples here?}
\sr{This might be interesting, and it is also related to sample complexity bounds in semi-supervised learning or active learning communities}. 
%
Second, the nature of the recovered decision boundary is highly dependent on the choice of samples. 
%
For example, with the random choice of samples (second and third rows, first and third columns of the figure), the recovered decision boundaries do not faithfully reflect the ideal decision boundaries shown in the \figref{fig:ictx_convergence} (first column).
%
However, with the diverse sampling, the recovered decision boundaries classify the given datasets more accurately for a given labeled set size. 
%
This shows that the performance of the ICT-based semi-supervised models is related to the choice of samples we choose to label. 
%
\todo{We need to run ICT on CIFAR-10/ SVHN with different sampling strategies to further concretize this point.}








\begin{figure*}[t]
        \def \MINPAGE {0.31}
        \def \FIGSCALE {0.38}
        \def \LABELS {250}
        \def \CTWEIGHT {100}
	    \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar10_labels\LABELS_weight\CTWEIGHT_layer0_linearity.pdf}\\
                 {\small Layer 0}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar10_labels\LABELS_weight\CTWEIGHT_layer1_linearity.pdf}\\
                 {\small Layer 1}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar10_labels\LABELS_weight\CTWEIGHT_layer2_linearity.pdf}\\
                 {\small Layer 2}
        \end{center}
        \end{minipage}
        
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar10_labels\LABELS_weight\CTWEIGHT_layer3_linearity.pdf}\\
                 {\small Layer 3}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar10_labels\LABELS_weight\CTWEIGHT_layer4_linearity.pdf}\\
                 {\small Layer 4}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar10_labels\LABELS_weight\CTWEIGHT_layer5_linearity.pdf}\\
                 {\small Layer 5}
        \end{center}
        \end{minipage}
        
\caption{Linearity propagation in different layers for CIFAR-10 with \LABELS\ labeled examples and consistency weight of \CTWEIGHT. ERM and mixup refer to the cases where only supervised loss is used. $\ictx_K$ refer to a setup where the ICT loss with $K$ mixup points are used as unsupervised loss. The supervised loss with the ICT does not use mixup.}
\label{fig:cifar10_labels250_cw100_linearity}
\end{figure*}

\begin{figure*}[t]
        \def \MINPAGE {0.31}
        \def \FIGSCALE {0.38}
        \def \LABELS {2000}
        \def \CTWEIGHT {100}
	    \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar10_labels\LABELS_weight\CTWEIGHT_layer0_linearity.pdf}\\
                 {\small Layer 0}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar10_labels\LABELS_weight\CTWEIGHT_layer1_linearity.pdf}\\
                 {\small Layer 1}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar10_labels\LABELS_weight\CTWEIGHT_layer2_linearity.pdf}\\
                 {\small Layer 2}
        \end{center}
        \end{minipage}
        
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar10_labels\LABELS_weight\CTWEIGHT_layer3_linearity.pdf}\\
                 {\small Layer 3}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar10_labels\LABELS_weight\CTWEIGHT_layer4_linearity.pdf}\\
                 {\small Layer 4}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar10_labels\LABELS_weight\CTWEIGHT_layer5_linearity.pdf}\\
                 {\small Layer 5}
        \end{center}
        \end{minipage}
        
\caption{Linearity propagation in different layers for CIFAR-10 with \LABELS\ labeled examples and consistency weight of \CTWEIGHT. ERM and mixup refer to the cases where only supervised loss is used. $\ictx_K$ refer to a setup where the ICT loss with $K$ mixup points are used as unsupervised loss. The supervised loss with the ICT does not use mixup.}
\label{fig:cifar10_labels2000_cw100_linearity}
\end{figure*}

\begin{figure*}[t]
        \def \MINPAGE {0.31}
        \def \FIGSCALE {0.38}
        \def \LABELS {4000}
        \def \CTWEIGHT {100}
	    \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar10_labels\LABELS_weight\CTWEIGHT_layer0_linearity.pdf}\\
                 {\small Layer 0}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar10_labels\LABELS_weight\CTWEIGHT_layer1_linearity.pdf}\\
                 {\small Layer 1}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar10_labels\LABELS_weight\CTWEIGHT_layer2_linearity.pdf}\\
                 {\small Layer 2}
        \end{center}
        \end{minipage}
        
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar10_labels\LABELS_weight\CTWEIGHT_layer3_linearity.pdf}\\
                 {\small Layer 3}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar10_labels\LABELS_weight\CTWEIGHT_layer4_linearity.pdf}\\
                 {\small Layer 4}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar10_labels\LABELS_weight\CTWEIGHT_layer5_linearity.pdf}\\
                 {\small Layer 5}
        \end{center}
        \end{minipage}
        
\caption{Linearity propagation in different layers for CIFAR-10 with \LABELS\ labeled examples and consistency weight of \CTWEIGHT. ERM and mixup refer to the cases where only supervised loss is used. $\ictx_K$ refer to a setup where the ICT loss with $K$ mixup points are used as unsupervised loss. The supervised loss with the ICT does not use mixup.}
\label{fig:cifar10_labels4000_cw100_linearity}
\end{figure*}

\begin{figure*}[t]
        \def \MINPAGE {0.31}
        \def \FIGSCALE {0.38}
        \def \LABELS {250}
        \def \CTWEIGHT {100}
	    \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/svhn_labels\LABELS_weight\CTWEIGHT_layer0_linearity.pdf}\\
                 {\small Layer 0}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/svhn_labels\LABELS_weight\CTWEIGHT_layer1_linearity.pdf}\\
                 {\small Layer 1}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/svhn_labels\LABELS_weight\CTWEIGHT_layer2_linearity.pdf}\\
                 {\small Layer 2}
        \end{center}
        \end{minipage}
        
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/svhn_labels\LABELS_weight\CTWEIGHT_layer3_linearity.pdf}\\
                 {\small Layer 3}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/svhn_labels\LABELS_weight\CTWEIGHT_layer4_linearity.pdf}\\
                 {\small Layer 4}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/svhn_labels\LABELS_weight\CTWEIGHT_layer5_linearity.pdf}\\
                 {\small Layer 5}
        \end{center}
        \end{minipage}
        
\caption{Linearity propagation in different layers for SVHN with \LABELS\ labeled examples and consistency weight of \CTWEIGHT. ERM and mixup refer to the cases where only supervised loss is used. $\ictx_K$ refer to a setup where the ICT loss with $K$ mixup points are used as unsupervised loss. The supervised loss with the ICT does not use mixup.}
\label{fig:svhn_labels250_cw100_linearity}
\end{figure*}

\begin{figure*}[t]
        \def \MINPAGE {0.31}
        \def \FIGSCALE {0.38}
        \def \LABELS {2000}
        \def \CTWEIGHT {100}
	    \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/svhn_labels\LABELS_weight\CTWEIGHT_layer0_linearity.pdf}\\
                 {\small Layer 0}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/svhn_labels\LABELS_weight\CTWEIGHT_layer1_linearity.pdf}\\
                 {\small Layer 1}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/svhn_labels\LABELS_weight\CTWEIGHT_layer2_linearity.pdf}\\
                 {\small Layer 2}
        \end{center}
        \end{minipage}
        
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/svhn_labels\LABELS_weight\CTWEIGHT_layer3_linearity.pdf}\\
                 {\small Layer 3}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/svhn_labels\LABELS_weight\CTWEIGHT_layer4_linearity.pdf}\\
                 {\small Layer 4}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/svhn_labels\LABELS_weight\CTWEIGHT_layer5_linearity.pdf}\\
                 {\small Layer 5}
        \end{center}
        \end{minipage}
        
\caption{Linearity propagation in different layers for SVHN with \LABELS\ labeled examples and consistency weight of \CTWEIGHT. ERM and mixup refer to the cases where only supervised loss is used. $\ictx_K$ refer to a setup where the ICT loss with $K$ mixup points are used as unsupervised loss. The supervised loss with the ICT does not use mixup.}
\label{fig:svhn_labels2000_cw100_linearity}
\end{figure*}

\begin{figure*}[t]
        \def \MINPAGE {0.31}
        \def \FIGSCALE {0.38}
        \def \LABELS {4000}
        \def \CTWEIGHT {100}
	    \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/svhn_labels\LABELS_weight\CTWEIGHT_layer0_linearity.pdf}\\
                 {\small Layer 0}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/svhn_labels\LABELS_weight\CTWEIGHT_layer1_linearity.pdf}\\
                 {\small Layer 1}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/svhn_labels\LABELS_weight\CTWEIGHT_layer2_linearity.pdf}\\
                 {\small Layer 2}
        \end{center}
        \end{minipage}
        
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/svhn_labels\LABELS_weight\CTWEIGHT_layer3_linearity.pdf}\\
                 {\small Layer 3}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/svhn_labels\LABELS_weight\CTWEIGHT_layer4_linearity.pdf}\\
                 {\small Layer 4}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/svhn_labels\LABELS_weight\CTWEIGHT_layer5_linearity.pdf}\\
                 {\small Layer 5}
        \end{center}
        \end{minipage}
        
\caption{Linearity propagation in different layers for SVHN with \LABELS\ labeled examples and consistency weight of \CTWEIGHT. ERM and mixup refer to the cases where only supervised loss is used. $\ictx_K$ refer to a setup where the ICT loss with $K$ mixup points are used as unsupervised loss. The supervised loss with the ICT does not use mixup.}
\label{fig:svhn_labels4000_cw100_linearity}
\end{figure*}

\begin{figure*}[t]
        \def \MINPAGE {0.31}
        \def \FIGSCALE {0.38}
        \def \LABELS {100}
        \def \CTWEIGHT {100}
	    \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar100_labels\LABELS_weight\CTWEIGHT_layer0_linearity.pdf}\\
                 {\small Layer 0}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar100_labels\LABELS_weight\CTWEIGHT_layer1_linearity.pdf}\\
                 {\small Layer 1}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar100_labels\LABELS_weight\CTWEIGHT_layer2_linearity.pdf}\\
                 {\small Layer 2}
        \end{center}
        \end{minipage}
        
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar100_labels\LABELS_weight\CTWEIGHT_layer3_linearity.pdf}\\
                 {\small Layer 3}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar100_labels\LABELS_weight\CTWEIGHT_layer4_linearity.pdf}\\
                 {\small Layer 4}
        \end{center}
        \end{minipage}\hfill
        \begin{minipage}[t]{\MINPAGE\textwidth}
        \begin{center}
                \includegraphics[scale=\FIGSCALE]{plots/linearity_new/cifar100_labels\LABELS_weight\CTWEIGHT_layer5_linearity.pdf}\\
                 {\small Layer 5}
        \end{center}
        \end{minipage}
        
\caption{Linearity propagation in different layers for CIFAR-100 with \LABELS\ labeled examples and consistency weight of \CTWEIGHT. ERM and mixup refer to the cases where only supervised loss is used. $\ictx_K$ refer to a setup where the ICT loss with $K$ mixup points are used as unsupervised loss. The supervised loss with the ICT does not use mixup.}
\label{fig:cifar100_labels1000_cw100_linearity}
\end{figure*}


==> related_work.tex <==
\section{Related Work} \label{sec:rel_work}

\ac{Maybe we can reduce some of the details around the methods that we are citing here.}

Mixup regularization is used in both supervised and semi-supervised setups to learn \emph{better network representations}.
%
In the context of supervised learning, the representations learned through mixup regularization are shown to improve generalization of the network and also its robustness to corrupt labels~\citep{Zhang2017}. This work showed that random sampling of mixup pairs produces the best results in comparison to other scenarios:  same class (SC) + random pairing, same class (SC) + k-nearest neighbor (kNN) pairing, and all class (AC) + kNN pairing. Concurrently, two other methods exploring the same idea were proposed~\citep{Inoue2018,Tokuzume2017}. 
%
Further, \citet{thulasidasan2020mixup} showed that mixup leads to improved calibration and predictive uncertainty of the network.
%

In the context of semi-supervised learning, mixup regularization, also known as interpolation consistency training (ICT), is shown to improve the performance of a learner significantly. Specifically, \citet{verma2019interpolation}, showed that mixup training encourages the consistency regularization which is an effective unsupervised learning signal explored in many works~\citep{sajjadi2016regularization,laine2016temporal,tarvainen2017mean,miyato2018virtual}. Other related methods include mixmatch~\cite{berthelot2019mixmatch} that rely on mixing labeled and unlabeled samples, and methods relying on pseudo-labels~\cite{sohn2020fixmatch} and data augmentation~\cite{xie2020unsupervised}.

%In ~\cite{Zhang2017}, it was first shown that convex combinations of pairs of examples and their labels can be used for training networks with improved generalization and robustness to corrupt labels. Their paper argues that the linear behavior reduces the undesirable oscillations outside the training data and is also a good inductive bias as per Occam’s razor. Mixup can be seen as a vicinal risk minimization (VRM) principle~\citep{Chapelle2000VicinalRM} technique, where we generate and train models from the samples near the the vicinity of training dataset~\citep{Chapelle2000VicinalRM}. This work showed that random sampling of mixup pairs produces the best results in comparison to other scenarios:  same class (SC) + random pairing, same class (SC) + k-nearest neighbor (kNN) pairing, and all class (AC) + kNN pairing. Concurrently, two other methods exploring the same idea were proposed~\citep{Inoue2018,Tokuzume2017}. 

%In \cite{thulasidasan2020mixup} introduces expected calibration error (ECE) and overconfidence error (OE) based on defining different calibration bins and estimating accuracy and confidence measures for these bins. If the gap between confidence and accuracy is high, we can have overconfidence error. 

There has been several methods extending mixup beyond simple convex combination of images and labels. For example, SuperMix~\cite{dabouei2020supermix} uses mixing masks and the image mixing is done based on the salient features in the image. In CutMix~\cite{yun2019cutmix}, we cut and paste patches among training samples and the area of the patches determine the mixup ratio for the output labels. In a long-tailed setting, remix~\cite{chou_remix_2020} focuses on doing mixup without using the same mixup ratio for both in the image space and output space.


%{\bf Image-specific mixup.} While the general idea of mixup focuses on convex combinations of whole images, SuperMix~\cite{dabouei2020supermix} uses mixing masks and the image mixing is done based on the salient features in the image. This also extends the task of mixing more than two images. The mixing masks are solved through an optimization algorithm that ensures that the generated images lie close to the manifold of training images, and sparsity is enforced such that the pixels in the mixup image usually comes from a single image. A teacher model was used to find the salient pixels in the original image, and the performance of SuperMix degrades when applied on more than 2 images on CIFAR100, and achieved the best results while mixing three images on ImageNet dataset. In CutMix~\cite{yun2019cutmix}, we cut and paste patches among training samples and the area of the patches determine the mixup ratio for the output labels. Image-transformations such as rotation and translation are combined with mixup to produce semantically meaningful nearby images in AugMix~\cite{hendrycks2020augmix}.

%{\bf Mixup for unbalanced datasets} In a long-tailed setting, remix~\cite{chou_remix_2020} focuses on doing mixup without using the same mixup ratio for both in the image space and output space. For example, let us consider a scenario where butterfly images correspond to tail classes and yellow-flower corresponds to head classes. While mixing butterfly and yellow-flower images in a 7:3 ratio, the output label could just be butterfly label. The main idea of remix is to relax the constraint of using same mixup ratio in both the image space and label space, and use higher mixup label coefficient for the tail classes. Note that even in cite~\citep{Inoue2018} (one of the first papers on mixup), two images were mixed to get an average and the label of only the first image was used while training. 

%{\bf Mixup for semi-supervised learning (SSL)} SSL is a class of wekly-supervised methods where we utilize a small amount of labeled data along with a large number of unlabeled samples. In \cite{verma2019interpolation}, the predictions of the interpolations of unlabeled samples are matches with the interpolations of their predictions. In Mixmatch~\cite{berthelot2019mixmatch}, we predict low-entropy labels for unlabeled data points and design mixing strategies with other labeled and unlabeled data points using MixUp to achieve semi-supervised learning. The general idea of FixMatch~\cite{sohn2020fixmatch} is closely related to Mixmatch, but much simpler. Here, we first generate pseudo-labels for weak augmentations of unlabeled data points and the pseudo-labels are used only if the model confidence is high. Next, we match the predictions of the strong augmentations of the same image with the pseudo-labels from weak augmentations. A related algorithm for semi-supervised learning is unsupervised data augmentation (UDA), where consistency is enforced on the predictions from data augmented unlabeled samples after sharpening their predictions~\cite{xie2020unsupervised}. In addition, UDA selects samples where the model is very confident and only considers the loss from confident samples in the minibatch. 

Beyond images, mixup has been extended to sound signals~\citep{Tokuzume2017} and sentence classification~\citep{guo2019mixup}

%{\bf Beyond Images.} One of the first papers on mixup in fact considered mixing sound signals~\citep{Tokuzume2017}. This work used random mixing ratio to combine input sound signals and their corresponding mixed outputs were used in training. Mixup was used for CNN and LSTM-based sentence classification tasks~\citep{guo2019mixup}.


==> todo.tex <==
\section{TODO}

\begin{itemize}
    \item All TODO comments refer to the experiments that we need to run. 
    \item Convert all png files to pdf.
\end{itemize}
